Path convergence of Markov chains on large graphs

We consider two classes of natural stochastic processes on finite unlabeled graphs. These are Euclidean stochastic optimization algorithms on the adjacency matrix of weighted graphs and a modified version of the Metropolis MCMC algorithm on stochastic block models over unweighted graphs. In both cases we show that, as the size of the graph goes to infinity, the random trajectories of the stochastic processes converge to deterministic curves on the space of measure-valued graphons. Measure-valued graphons, introduced by Lov\'{a}sz and Szegedy in \cite{lovasz2010decorated}, are a refinement of the concept of graphons that can distinguish between two infinite exchangeable arrays that give rise to the same graphon limit. We introduce new metrics on this space which provide us with a natural notion of convergence for our limit theorems. This notion is equivalent to the convergence of infinite-exchangeable arrays. Under suitable assumptions and a specified time-scaling, the Metropolis chain admits a diffusion limit as the number of vertices go to infinity. We then demonstrate that, in an appropriately formulated zero-noise limit, the stochastic process of adjacency matrices of this diffusion converges to a deterministic gradient flow curve on the space of graphons introduced in\cite{Oh2023}. A novel feature of this approach is that it provides a precise exponential convergence rate for the Metropolis chain in a certain limiting regime. The connection between a natural Metropolis chain commonly used in exponential random graph models and gradient flows on graphons, to the best of our knowledge, is new in the literature as well.

==> figures/finite_NN.tex <==
\def\layersep{2cm}

\begin{figure}
    \centering
    \begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=green!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
    \tikzstyle{annot} = [text width=4em, text centered]

    \def\inp{4}
    \def\hone{5}
    \def\hi{4}
    \def\hipone{5}
    \def\hb{3}
    
    \foreach \name / \y in {1,...,\inp}
        \node[input neuron] (I-\name) at (0,-\y) {};

    \foreach \name / \y in {1,...,\hone}
        \path[yshift= (\hone-\inp)*0.5 cm]
            node[hidden neuron] (H1-\name) at (\layersep,-\y cm) {};

    \path[yshift=0cm]
    node[] (dots1) at (1.5*\layersep,-2.5 cm) {$\cdots$};

    \foreach \name / \y in {1,...,\hi}
        \path[yshift=(\hi-\inp)*0.5cm]
            node[hidden neuron] (Hi-\name) at (2*\layersep,-\y cm) {};

    \foreach \name / \y in {1,...,\hipone}
        \path[yshift=(\hipone-\inp)*0.5cm]
            node[hidden neuron] (Hipone-\name) at (3*\layersep,-\y cm) {};

    \path[yshift=0cm]
    node[] (dots1) at (3.5*\layersep,-2.5 cm) {$\cdots$};

    \foreach \name / \y in {1,...,\hb}
        \path[yshift=(\hb-\inp)*0.5cm]
            node[hidden neuron] (Hb-\name) at (4*\layersep,-\y cm) {};

    \node[output neuron,pin={[pin edge={->}]right:$\hat{y}(x_0)$}] (O) at (5*\layersep,-2.5 cm) {};

    \foreach \source in {1,...,\inp}
        \foreach \dest in {1,...,\hipone}
            \path (I-\source) edge (H1-\dest);

    \foreach \source in {1,...,\hi}
        \foreach \dest in {1,...,\hipone}
            \path (Hi-\source) edge (Hipone-\dest);

    \foreach \source in {1,...,\hb}
        \path (Hb-\source) edge (O);

    \node[annot,above of=I-1, node distance=1cm] (i) {$x_0$};
    \node[annot,above of=H1-1, node distance=1cm] (h1) {$x_1$};
    \node[annot,above of=Hi-1, node distance=1cm] (h2) {$x_i$};
    \node[annot,above of=Hipone-1, node distance=1cm] (h2) {$x_{i+1}$};
    \node[annot,above of=Hb-1, node distance=1cm] (hb) {$x_b$};
    % \node[annot,above of=O, node distance=1cm] (o) {Output layer};
    
    \node[annot,below of=I-\inp, node distance=1cm] (di) {$d_0$};
    \node[annot,below of=H1-\hone, node distance=1cm] (dh1) {$d_1$};
    \node[annot,below of=Hi-\hi, node distance=1cm] (dh2) {$d_i$};
    \node[annot,below of=Hipone-\hipone, node distance=1cm] (dh2) {$d_{i+1}$};
    \node[annot,below of=Hb-\hb, node distance=1cm] (dhb) {$d_b$};
\end{tikzpicture}
    \caption{Finite width Neural Network with multiple hidden layers.}
    \label{fig:finite_NN}
\end{figure}
